Maximum Causal Entropy Inverse Constrained Reinforcement Learning

When deploying artificial agents in real-world environments where they interact with humans, it is crucial that their behavior is aligned with the values, social norms or other requirements of that environment. However, many environments have implicit constraints that are difficult to specify and transfer to a learning agent. To address this challenge, we propose a novel method that utilizes the principle of maximum causal entropy to learn constraints and an optimal policy that adheres to these constraints, using demonstrations of agents that abide by the constraints. We prove convergence in a tabular setting and provide an approximation which scales to complex environments. We evaluate the effectiveness of the learned policy by assessing the reward received and the number of constraint violations, and we evaluate the learned cost function based on its transferability to other agents. Our method has been shown to outperform state-of-the-art approaches across a variety of tasks and environments, and it is able to handle problems with stochastic dynamics and a continuous state-action space.

==> background.tex <==
\section{Maximum entropy}
Probability of a trajectory in a deterministic MDP under the maximum entropy model \cite{ziebart2008maximum}:
\begin{equation}
    p_{\mathcal{M}}(\tau) = \dfrac{\textrm{exp}(r(\tau))}{Z_{\mathcal{M}}}
\end{equation}
With the partition function
\begin{equation}
    Z_{\mathcal{M}} = \int \textrm{exp}(r(\tau))
\end{equation}
The probability of a trajectory under a constrained MDP:
\begin{equation}
    p_{\mathcal{M^{\mathcal{C}}}}(\tau) = \dfrac{\textrm{exp}(r(\tau))}{Z_{\mathcal{M}}}\mathbb{1}^{\mathcal{M}^{\mathcal{C}}}(\tau)
\end{equation}
partition function:
\begin{equation}
    Z_{\mathcal{M}^{\mathcal{C}}} = \int \textrm{exp}(r(\tau))\zeta(\tau)
\end{equation}
The probability of a set of trajectories $\mathcal{D}$ given a set of constraints:
\begin{equation}
    p_{\mathcal{M}}(\mathcal{D} \mid \mathcal{C}) = \dfrac{1}{(Z_{\mathcal{M}^{\mathcal{C}}})^{N}}\prod_{i=1}^{N} \textrm{exp}(r(\tau^{(i)})) \mathbb{1}^{\mathcal{M}^{\mathcal{C}}}(\tau^{(i)}).
\end{equation}
Consider the log likelihood of the set of constraints.
\begin{equation}
    \mathcal{L}(\mathcal{C}) = \dfrac{1}{N}\log p_{\mathcal{M}}(\mathcal{D} \mid \mathcal{C})
\end{equation}
Let's use a binary classifier $\zeta_{\theta}$ parameterized with $\theta$. We want $\zeta_{\theta}(s_t, a_t)$ to be one if $(s_t, a_t)$ is not in $\mathcal{C}$.
Since the set of constraints is determined by the parameters $\theta$:
\begin{gather}
    \mathcal{L}(\mathcal{C}) = \mathcal{L}(\theta) = \dfrac{1}{N} \sum^{N}_{i=1} \left[ r(\tau^{(i)}) + \log \zeta_{\theta}(\tau^{(i)}) \right] \\ - \log \int \textrm{exp}(r(\tau))\zeta_{\theta}(\tau)d \tau
\end{gather}
Taking the gradient gives us:
\begin{equation}
    \nabla_{\theta}\mathcal{L}(\theta) = \dfrac{1}{N}\sum^{N}_{i=1} \nabla_{\theta} \log \zeta_{\theta}(\tau^{(i)}) - \mathbb{E}_{\tau \sim \pi_{\mathcal{M}^{\zeta_{\theta}}}}\left[ \nabla_{\theta} \log \zeta_{\theta}(\tau) \right]
\end{equation}
Using a sample based approximation for the right-hand term:
\begin{equation}
    \nabla_{\theta}\mathcal{L}(\theta) \approx \dfrac{1}{N}\sum^{N}_{i=1} \nabla_{\theta} \log \zeta_{\theta}(\tau^{(i)}) - \dfrac{1}{M}\sum^{M}_{j=1}\nabla_{\theta} \log \zeta_{\theta}(\hat{\tau}^{(j)})
\end{equation}
The constraint net is alternately trained with the policy.
The policy is parameterized with parameters $\psi$ and trained using the following objective:
\begin{equation}
    \min_{\lambda \geq 0} \max_{\psi} J(\pi^{\psi}) + \dfrac{1}{\beta}\mathcal{H}(\pi^{\psi}) - \lambda(\mathbb{E}_{\tau \sim \pi^{\psi}}[1-\zeta_{\theta}(\tau)] - \alpha) 
\end{equation}
When inspecting the code of Malik et al. \cite{malik2021inverse}, the loss on the actor (parameterized with $\psi$) is calculated as follows (I think when taking into account the other loss terms this can indeed be reduced to the equation above from the papaer):
\begin{equation}
    L(\psi) = \mathbb{E}[\log \pi_{\psi}(a_t \mid s_t)(\lambda \hat{A}_t^C - \hat{A}_t^R)]
\end{equation}
Here, $\hat{A}_t^C$ and $\hat{A}_t^R$ represent the estimated advantage on the cost and reward respectively.
These advantages are estimated using GAE \cite{schulman2015high}.
We can define the total estimated advantage as:
\begin{equation}
    \label{eq:advantage_def}
    \hat{A} = \lambda \hat{A}_t^C - \hat{A}_t^R
\end{equation}
\section{Maximum causal entropy}
The model of maximum entropy does only exactly holds for deterministic environments. Gleave et al. \cite{gleave2022primer} even theorize applying the maximum entropy principle in stochastic environments induces risk-seeking behavior.
In stochastic MDP's the principle of maximum causal entropy \cite{ziebart2010modeling} should be applied.
\begin{equation}
    p_{\mathcal{M}}(s_t,a_t) = \textrm{exp}(Q_t^{\textrm{soft}}(s_t, a_t)-V_t^{\textrm{soft}}(s_t)).
\end{equation}
Ziebart et al. propose a softened version of value iteration \cite{bellman1957markovian} to calculate $Q{\textrm{soft}}_{t}(s_t, a_t)$ and $V{\textrm{soft}}_{t}(s_t)$: 
\begin{equation}
    Q^{\textrm{soft}}_t(s_t, a_t) = r(s_t, a_t) + \mathbb{E}_{s_{t+1}}(V^{\textrm{soft}}_{t+1}(s_{t+1}))
\end{equation}
\begin{equation}
    V^{\textrm{soft}}_{t}(s_t)=\log \sum_{a_t}\textrm{exp}(Q^{\textrm{soft}}_t(s_t, a_t))
\end{equation}
\begin{equation}
    V^{\textrm{soft}}_{t}(s_t)=\textrm{soft}\max_{a_t}(Q^{\textrm{soft}}_t(s_t, a_t))
\end{equation}
The probability of a trajectory is defined as:
\begin{equation}
    p_{\mathcal{M}}(\tau) = \prod_{t=1}^{T} \textrm{exp}(Q_t^{\textrm{soft}}(s_t, a_t)-V_t^{\textrm{soft}}(s_t))).
\end{equation}
Under a constrained MDP this becomes:
\begin{equation}
    p_{\mathcal{M}^{\mathcal{C}}}(\tau) = \prod_{t=1}^{T} \textrm{exp}(Q_t^{\textrm{soft}}(s_t, a_t)-V_t^{\textrm{soft}}(s_t))\mathbb{1}^{\mathcal{M}^{\mathcal{C}}}(\tau).
\end{equation}
The probability of a set of trajectories $\mathcal{D}$ is given by:
\begin{equation}
    p_{\mathcal{M}}(\mathcal{D} \mid \mathcal{C}) = \mathbb{E}_{\mathcal{D}} \prod_{t=1}^{T} \textrm{exp}(Q_t^{\textrm{soft}}(s_t, a_t)-V_t^{\textrm{soft}}(s_t))\mathbb{1}^{\mathcal{M}^{\mathcal{C}}}(\tau).
\end{equation}
We, again, define the log likelihood and use a binary classifier $\zeta_{\theta}$:
\begin{gather}
    \label{eq:log_likelihood1}
    \mathcal{L}(\mathcal{C}) = \mathcal{L}(\theta) = \mathbb{E}_{\mathcal{D}} \sum_{t=1}^{T} Q_t^{\textrm{soft}}(s_t, a_t)-V_t^{\textrm{soft}}(s_t)+ \log \zeta_{\theta}(s_t, a_t)
\end{gather}
The subtraction $Q_t^{\textrm{soft}}(s_t, a_t)-V_t^{\textrm{soft}}(s_t)$ is referred to in the literature as the advantage: how good is the chosen action $a_t$ in state $s_t$ compared to the average.
When using an actor-critic method (e.g. PPO), the value function $V(s_t)$ is parameterized by the critic network.
Since
\begin{equation}
    Q(s_t, a_t) = \textbb{E}[r_{t+1} + \gamma V(s_{t+1})] 
\end{equation}
equation \ref{eq:log_likelihood1} becomes
\begin{gather}
    = \mathcal{L}(\theta) = \mathbb{E}_{\mathcal{D}} \sum_{t=1}^{T} r_{t+1} + \gamma V(s_{t+1})-V_t(s_t)+ \log \zeta_{\theta}(s_t, a_t)
\end{gather}
We can train our constraint net using gradient ascent, this will make sure all demonstrated trajectories are classified as valid while trajectories which have a higher advantage are exponentially more likely.
This intuitively makes sense as the network is punished when an expert interaction is worse than average.
\\
Another possibility is using the advantage definition applied in our forward step (equation \ref{eq:advantage_def}).
The log likelihood of $\theta$ becomes:
\begin{align}
    \mathcal{L}(\theta) &= \mathbb{E}_{\mathcal{D}} \sum_{t=1}^{T} \hat{A} + \log \zeta_{\theta}(s_t, a_t) \\
    &= \mathbb{E}_{\mathcal{D}} \sum_{t=1}^{T} \lambda \hat{A}_t^C - \hat{A}_t^R  + \log \zeta_{\theta}(s_t, a_t)
\end{align}
When using the principle of causal entropy we do not need to sample nominal trajectories.
\\
Instead of learning a policy using the soft value iteration algorithm proposed by Ziebart et al. We use PPO and add the causal entropy to the loss to get the maximum causal entropy policy.


==> method.tex <==
We generate expert demonstrations, following a set of ground truth consraints, by sampling from an expert policy trained with Reward Constrained Policy Optimization (RCPO) \cite{tessler2018reward}.
\subsection{Constrained Reinforcement Learning}
\subsection{Inverse Constrained Reinforcement Learning}
We build on the principle of maximum likelihood constraint inference \cite{scobee2019maximum} to infer constraints from expert trajectories and adopt the sample-based approximation proposed by Malik et al. \cite{malik2021inverse}.
We assume a set of expert trajectories $\mathcal{T}$ sampled from an unknown expert policy $\pi^*$ is available.
This expert operates in the constrained MDP $\mathcal{M}^{C^*}$, where $C^*$ represents the ground-truth set of constraints.
The goal of our work is to learn a set of logical rules which classify state-action pairs as constraint or valid.
To enable the integration of a logic component with popular reinforcement learning techniques based on deep learning, we adopt a neuro-symbolic approach called logical neural networks (LNN) \cite{riegel2020logical}.
\subsection{Logical Constraint Net}
We adopt a real-valued logic where each proposition and the output of all neurons take values in $[0,1]$.
To facilitate interpretability, a threshold $\alpha$ is defined which maps a continuous truth value to \verb|True| or \verb|False|.
Values larger or equal to $\alpha$ are considered \verb|True|, values smaller than $\alpha$ are considered \verb|False|.
The output $y$ of a logical neuron is computed by the activation function $\sigma$ of the dot-product of the weight vector $W$ and the input vector $x$: $y=\sigma(Wx)$.
We distinguish two types of neurons corresponding with the logical conjunction (AND) and the logical disjunction (OR).
The activation function $\sigma$ is defined as a sigmoid function shifted along the x-axis with a value $x_T$.
$x_T$ is a weight dependent threshold which controls when the neuron is activated.
To obtain interpretable weights we augment the sigmoid function with a temperature variable $\tau$ which controls the steepness of the function.
When $\tau$ approaches infinity the sigmoid becomes a Heaviside step function and the weights can be interpreted as an attention vector which selects a portion of the inputs.
The activation function is defined as:
\begin{equation}
    \sigma(x) = \dfrac{1}{1+e^{-\tau(x-x_t)}}.
\end{equation}
For a conjunction neuron $x_T$ is calculated as the product of $\alpha$ and the sum of all weights:
\begin{equation}
    x_T = \alpha \sum w_i.
\end{equation}
For a disjunction neuron $x_T$ is calculated as the product of $\alpha$ and the maximum weight:
\begin{equation}
    x_T = \alpha w_{\textrm{max}}.
\end{equation}
\subsection{Network Pruning}
For a conjunction neuron, only weights $w_k$ for which $\sum w_i - \alpha w_k \leq x_T$ are kept, all other connections are pruned.
Evaluating this expression reveals if an input affects the output of the neuron. 
If the input $x_k$ is true, its value is equal or greater than $\alpha$.
By subtracting $\alpha w_k$ from $\sum w_i$, we simulate what would happen to the output if we ignore this input.
If the output would still be equal or greater than $x_T$, we can conclude this feature can be ignored by the current neuron.
By rewriting the above expression, we obtain a weight threshold value $k$, i.e. every weight below this value can be pruned without changing the behavior of the neuron.
\begin{equation}
    k = \dfrac{1-\alpha}{\alpha}\sum w_i 
\end{equation}
For the disjunction a similar threshold can be computed:
\begin{equation}
    k = \alpha w_{\textrm{max}}
\end{equation}

==> related_work.tex <==
In preliminary work on ICRL, \citet{chou2018learning} learn constraints given a nominal model of the environment and a set of expert demonstrations.
Constraints are defined as a subset of the feature space for which a higher reward is obtained compared to the expert demonstrations.
\citet{scobee2019maximum} extend this idea and adapt the principle of maximum entropy which enables ranking the likelihood of possible constraints.
\citet{glazier2022learningbehavioral} extend this to learning probabilities of constraints and \citet{papadimitriou2021bayesian} introduce a Bayesian approach to infer a posterior distribution over constraints.
%Probability mass is assigned to constraints which are consistent with the demonstrations and have support in the prior.
Expressing constraints as probabilities enables agents to incorporate the uncertainty of constraints in their policy.
All mentioned methods learn a discrete set of constraints and assume the state-action space is discrete and has a limited size.
To scale ICRL to problems with continuous dynamics \citet{stocking2021discretizingdynamics} proposed to extract a tabular representation of the state space and use this approximation to learn constraints.
An alternative approach \cite{malik2021inverse} 
(mentioned earlier as ME-ICRL) introduces an approximation of the work of \citet{scobee2019maximum} which uses a neural network to parameterize a cost function instead of learning a discrete set of constraints.
This also extends the applicability of ICRL to problems with unknown transition dynamics.
\citet{liu2022benchmarking} introduce variational ICRL (VME-ICRL) and define an evidence lower bound objective to learn a cost function modeled as a $\beta$-distribution.
All mentioned works build on the principle of maximum entropy restricting their applicability to problems with deterministic dynamics.
One approach, also building on the principle of maximum causal entropy, was proposed but only considers discrete state-action spaces with known transition dynamics \cite{mcpherson2021maximum}.
In this work, we fill the gap of a method which holds for stochastic dynamics but also scales to complex environments with a continuous state-action space and unknown transition dynamics.
An important, but subtle, difference between the maximum entropy methods (ME-ICRL and VME-ICRL) and MCE-ICRL is that for the latter the Lagrange multiplier $\lambda$ is part of the cost network.
In the ME methods, a cost function is learned during the backward pass and used by a constrained optimization method (e.g. \cite{tessler2018reward}) to update the nominal policy.
Another difference between these methods and ours, is that we propose the objective from scratch instead of adapting an IRL objective to the ICRL case.
% VME-ICRL takes the effect of stochastic environment dynamics into account by learning a distribution over constraints [Is this enough, assess this based on results of experiments].
%Our logic neurons are inspited by logical neural networks (LNN) \cite{riegel2020logical}.
%LNN's also use a threshold $\alpha$ to interpret continuous truth values and use a comparable activation function to constrain the weights of the logical neurons.
%However, their experiments are focused on reasoning and they do not validate the interpretability of the weights.
%LNN's also operate on truth bounds while for our use case, a single bound is more suitable.
%Our work builds on that of Malik et al. \cite{malik2021inverse} but replace standard fully connected constraint network with a logical network.
%Some work focuses on learning constraints in stochastic domains, i.e. soft constraints \cite{gaurav2022learning}.
%Another direction we would like to explore is extending our logic network from Boolean to signal temporal logic.
%This would enable learning constraints referring real valued temporal properties time (e.g. the distance between two agents should always be less than x).
%Papadimitriou et al. \cite{papadimitriou2021bayesian} propose a Bayesian approach to infer a posterior distribution over constraints.
%Probability mass is assigned to constraints which are consistent with the demonstrations and have support in the prior.
%Because the set of constraints is defined as a binary vector where each entry represents a single state, this method is only suited for problems with a relative small state space and constraints defined as single states which limits the scalability of the approach.
%They claim there method is able to cope with constraint violations in the expert demonstrations but this is not evaluated in experiments or theoretically proven.
%Glazier et al. \cite{glazier2022learningbehavioral} propose a method to learns probabilities of constraints (instead of penalties). This leverages comparison of constraints across different environments with different scales.
%The cost function is represented by the dot product of a learned vector and a hard-coded feature representation.
%This only facilitates learning linear cost functions w.r.t. the hard-coded feature representation.
%They extend the work of Scobee et al. \cite{scobee2019maximum} to environments with stochastic dynamics by defining the cost function over the set of transitions: $C: S \times A \times S \rightarrow \mathbb{R}$.
%Although experiments confirms this is a valid approach, the complexity  of the cost function is increased.
%In this work, we adopt the principle of maximum causal entropy to handle stochasticity such that a much more simple cost function over state-action pairs can be used.
%Their method assumes the state-action space is discrete hence it was only validated in a simple gridworld environment.
%Future work is required to scale this method to more complex problems.
%problem of stochasticity is solved by MCE.
%problem of continuous state spaces is solve by using a neural network.
